Towards Language-Augmented Multi-Agent Deep Reinforcement Learning

Most prior works on communication in multi-agent reinforcement learning have focused on emergent communication, which often results in inefficient and non-interpretable systems. Inspired by the role of language in natural intelligence, we investigate how grounding agents in a human-defined language can improve the learning and coordination of embodied agents. We propose a framework in which agents are trained not only to act but also to produce and interpret natural language descriptions of their observations. This language-augmented learning serves a dual role: enabling efficient and interpretable communication between agents, and guiding representation learning. We demonstrate that language-augmented agents outperform emergent communication baselines across various tasks. Our analysis reveals that language grounding leads to more informative internal representations, better generalization to new partners, and improved capability for human-agent interaction. These findings demonstrate the effectiveness of integrating structured language into multi-agent learning and open avenues for more interpretable and capable multi-agent systems.

==> tex/6.3-transferlearning.tex <==
\subsection{Transfer Learning}
\label{sec:XP_Transfer}

We conduct a transfer learning experiment to investigate how language helps for generalizing to new domains. We first pre-train all variants on a $12\times12$ version of Predator-Prey (see Appendix~\ref{app:PP12} for the training performance in this setting). Then, agents are put in the larger $18\times18$ Predator-Prey setting and trained again. Increasing the size of the environment induces a change in the observations functions and in the policy space. 

\paragraph{Results.} Figure~\ref{fig:Transfer} presents the results of the transfer experiment, starting with the agents initially trained in the lower dimension Predator-Prey setting ($12\times12$, see Annex for results) and transferred to the larger environment used earlier (predator-prey $18\times18$). A first consideration is that all methods strongly benefit from transfer learning, as illustrated by No-comm with transfer ending up being on par with \texttt{LAMARL} without transfer (results from Fig.~\ref{fig:Train}). Secondly, \texttt{LAMARL} retains its dominance and consistently outperforms all baselines after transfer, and even continues to improve beyond stabilization, unlike all baselines which both stabilize and retain the same ordering regarding performance attained. 

\begin{figure}
    \centering
     \includesvg[width=0.7\linewidth]{Figures/transfer.svg}
    \caption{Training performance on the transfer experiment, from Predator-Prey $12\times 12$ to Predator-Prey $18\times 18$ (7 runs each, with median and 95\% confidence interval). 
    % \texttt{LAMARL} agents achieve similar performance as \texttt{Oracle} agents, showing that they succeed in using the language properly. All other ablations are inferior, showing both the importance of grounding representations in language and the efficiency of language for communication.}
    }
    \label{fig:Transfer}
\end{figure}

